On Controllable Sparse Alternatives to Softmax

Converting an n-dimensional vector to a probability distribution over n objects is a commonly used component in many machine learning tasks like multiclass classification, multilabel classification, attention mechanisms etc. For this, several probability mapping functions have been proposed and employed in literature such as softmax, sum-normalization, spherical softmax, and sparsemax, but there is very little understanding in terms how they relate with each other. Further, none of the above formulations offer an explicit control over the degree of sparsity. To address this, we develop a unified framework that encompasses all these formulations as special cases. This framework ensures simple closed-form solutions and existence of sub-gradients suitable for learning via backpropagation. Within this framework, we propose two novel sparse formulations, sparsegen-lin and sparsehourglass, that seek to provide a control over the degree of desired sparsity. We further develop novel convex loss functions that help induce the behavior of aforementioned formulations in the multilabel classification setting, showing improved performance. We also demonstrate empirically that the proposed formulations, when used to compute attention weights, achieve better or comparable performance on standard seq2seq tasks like neural machine translation and abstractive summarization.

==> 6_related.tex <==
\section{Related Work} \label{sec:related}

% In the unusual situation where you want a paper to appear in the
% references without citing it in the main text, use \nocite
% \nocite{langley00}

% sparsemax \cite{martins2016}
% spherical softmax \cite{DBLP:journals/corr/BrebissonV15}
% projection onto simplex duchi \cite{Duchi:2008:EPL:1390156.1390191}
% sparse recovery under simplex \cite{DBLP:journals/corr/LiRS16}
% sparse and structured attention \cite{DBLP:journals/corr/NiculaeB17}
% diversity based attention \cite{diverseattn17}
% sparsity in RNN \cite{DBLP:journals/corr/NarangDSE17}
% gumbel softmax\cite{jang2016categorical}
% region sparsity and diversity for visual attention \cite{Wei-etal-NIPS16}
% structured attention networks \cite{DBLP:journals/corr/KimDHR17}
% exact gradient update for very large sparse targets\cite{DBLP:conf/nips/VincentBB15}
% neural easy-first taggers \cite{martins-kreutzer:2017:EMNLP2017}
% sparsity on statistical simplexes and diversity in social ranking \cite{pmlr-v39-sun14}

% sparse projections onto simplex \cite{DBLP:journals/corr/abs-1206-1529}
% sparsity for submodular data summarization \cite{DBLP:conf/nips/LindgrenWD16}
% memory sparse reads and writes \cite{DBLP:journals/corr/RaeHHDSWGL16}
% pytorch \cite{pytorch}
% LIME \cite{lime2016}
% right for the right reasons \cite{ijcai2017-371}
% mythos of interpretability \cite{mythos16}
% science of interpretability \cite{scienceinterpretability17}
% trading interpretability for accuracy \cite{tradeinteracc15}
% Moses \cite{Koehn2007}
% rationalizing neural predictions \cite{lei-barzilay-jaakkola:2016:EMNLP2016}
% sparse coding \cite{NIPS2006_2979}, sparse autoencoders\cite{Vincent:2010:SDA:1756006.1953039}, 
% visualizing neural models \cite{li-EtAl:2016:N16-12}
% sparse cnn \cite{sparsecnn2015}
% group sparse regularization for dnn \cite{Scardapane2017}
% lasso book \cite{hastielasso2015}
% sparse modelling with feature grouping \cite{Zhong2012}
% structured sparsity in dnn \cite{NIPS2016_6504}
% encoder decoder cho \cite{cho-EtAl:2014:EMNLP2014}
% deep sparse rectifier neural networks \cite{pmlr-v15-glorot11a}
% end-to-end memory networks \cite{NIPS2015_5846}
% neural turing machines \cite{DBLP:journals/corr/GravesWD14}
% review on multi label learning \cite{Zhang2014}
% neural turing machine with soft and hard addressing \cite{GulcehreCCB16}
% online and linear time monotonic attention \cite{RaffelLLWE17}
% hybrid of soft and hard attention \cite{shen18}
% monotonic chunkwise attention \cite{chiu17}
% alternative to softmax in RL \cite{AsadiL17}
% memory with wormhole \cite{GulcehreCB17}


% These are all approximations.
% one: Sampling based techniques
% two: hierarchical softmax
% three: Dropmax \cite{lee17}
\textcolor{red}{
\begin{itemize}
    \item Sparsity literature for variable or feature selection \cite{Bach:2011:OSP:2208224,hastielasso2015}. How this compares : sparse coding \cite{NIPS2006_2979}, deep sparse rectifier neural networks \cite{pmlr-v15-glorot11a}, sparse autoencoders \cite{Vincent:2010:SDA:1756006.1953039}, sparse DNNs \cite{NIPS2016_6504}, sparse RBMs, sparse RNNs \cite{DBLP:journals/corr/NarangDSE17}, sparse CNN \cite{sparsecnn2015}, sparse linear regression (LIME \cite{lime2016}) - sparsity at outputs \cite{martins2016,DBLP:journals/corr/NiculaeB17}, interpretability need \cite{scienceinterpretability17,lime2016,mythos16,ijcai2017-371,tradeinteracc15,lei-barzilay-jaakkola:2016:EMNLP2016}.
    \item Why sparsity is needed for probability distributions - for example interpretability/computational. Contrast with sampling based approximations: Dropmax \cite{lee17}, Sampled Softmax \cite{jean-al-acl2015}, alternative to softmax in RL \cite{AsadiL17}. These are exact approaches.
    \item need for more interpretable attention with controls/structure, region sparsity and diversity for visual attention \cite{Wei-etal-NIPS16}, diversity based attention \cite{diverseattn17}, sparsity on statistical simplexes and diversity in social ranking \cite{pmlr-v39-sun14}. structured attention + sparse attention existing works - no control over sparsity \cite{martins2016,DBLP:journals/corr/NiculaeB17,DBLP:journals/corr/KimDHR17}.
    \item literature around scale invariance and translation invariance \cite{DBLP:journals/corr/BrebissonV15}. need to motivate why it is important to look at and nobody as looked at this.
    \item Applications of other techniques for hard selection like gumbel-softmax/other heuristics for sparse reads and writes in memory networks \cite{GulcehreCCB16,GulcehreCB17,DBLP:journals/corr/RaeHHDSWGL16,shen18}.
\end{itemize}}
